Human Error Management in Requirements Engineering: Should We Fix the People, the Processes, or the Environment?

Context: Software development is human-centric and vulnerable to human error. Human errors are errors in the human thought process. To ensure software quality, practitioners must understand how to manage these human errors. Organizations often change the requirements engineering process to prevent human errors from occurring or to mitigate the harm caused when those errors do occur. While there are studies on human error management in other disciplines, research on the prevention and mitigation of human errors in software engineering, and requirements engineering specifically, are limited. The software engineering studies do not provide strong results about the types of changes that are most effective in requirements engineering. Objective: The goal of this paper is to develop a taxonomy of human error prevention and mitigation strategies based on data from requirements engineering professionals. Method: We performed a qualitative analysis of two practitioner surveys on requirements engineering practices to identify and classify strategies for the prevention and mitigation of human errors. Results: We organized the human error management strategies into a taxonomy based on whether they primarily affect People, Processes, or the Environment. Inside each high-level category, we further organized the strategies into low-level classes. More than 50% of the reported strategies require a change in Process, 23% require a change in Environment, 21% require a change in People, with the remaining 5% too ambiguous to classify. In addition, more than 50\% of the strategies focus on Management activities. Conclusions: The Human Error Management Taxonomy provides a systematic classification and organization of strategies for prevention and mitigation of human errors in requirements engineering. This systematic organization provides a foundation upon which research can build.

==> New_Results.tex <==
\subsubsection{\textit{Phase 2: Classification of Prevention and Mitigation Strategies}}

The goal of this phase was to classify each prevention and mitigation strategy into the high-level categories, the low-level categories, and the requirements activities defined during Phase 1.

\vspace{8pt}
\noindent
\textit{Step 1: Classify the prevention and mitigation strategies into the high-level classes}

We individually classified each prevention and mitigation strategy into the high-level classes defined in Step 1 of Phase 1.
To facilitate the process we randomly assigned the prevention and mitigation strategies into five batches of 40, 31, 36, 40, and 28 strategies.
%\changes{
%The first 4 batches consisted of unique strategies.
%}
Included in the last batch were 13 randomly selected prevention and mitigation strategies from the disagreed strategies of the first 4 batches to allow us to validate our earlier classification.
After individually classifying the strategies in each batch, we compared our results and discussed any disagreements to resolve them.
We identified 17 disagreements in the first batch, 13 in the second, 7 in the third, 8 in the fourth, and 8 in the fifth.
After discussing the disagreements, all three authors agreed on the final classification.
\begin{comment}
Figure~\ref{fig:PmClassification} illustrates our procedure for classifying the prevention and mitigation strategies into the high-level classes. 
\begin{figure}
  \centering
  \includegraphics[width=4.5in]{Figures/PMClassification.PNG}
  \caption{Classification of Prevention and Mitigation Strategies}
  \label{fig:PmClassification}
\end{figure}
\end{comment}

\vspace{8pt}
\noindent
\textit{Step 2: Classify the prevention and mitigation strategies into the low-level classes and requirements phases}

Using the results from Step 1 as a starting point, the first author classified the prevention and mitigation strategies into the low-level classes.
She also classified each strategy into the requirements engineering lifecycle phase that was impacted by the change.
Then, the other two authors reviewed the classification and noted any disagreements.
Similar to the way we performed Step 1, we divided the review process into 4 batches of 15, 30, 49, and 59 strategies respectively.
We had a total of 29 disagreements across all four batches, which we resolved through the discussion sessions.

\subsubsection{\textit{Phase 3: Discussion about Disagreements}}
As described above, this phase ran multiple times, concurrently with Phases 1 and 2.
After each classification activity, we had a discussion to resolve any disagreements.
These periodic discussions helped ensure we had a consistent and correct understanding of the classification approach.
At the end of each discussion, all authors reached agreement.

==> Tables/EnvTable.tex <==
 %\rotatebox{90}{
 \begin{tabular}{|p{.20\textwidth} | p{.65\textwidth} | p{.078\textwidth} | }
  \hline
\textbf{Environment} & \textbf{Description} & \textbf{Code} \\ 
  \hline
Addition of New Process, Tool or Approaches & Changes in Environment by introducing new approaches, tools or process in software development.For example, introduction of agile methodology or new quality assurance process & ANP \\
  \hline
Addition of Personnel & Changes in Environment by addition of personnel that are not generally involved to work on that sub process. Examples include requirement experts, end users, clients &  AP\\
  \hline
Internal & Addition of personnel who work for the organization performing the requirement activities. For example, developers, managers, requirement engineers, business analysts and so on. &  Int \\
  \hline
External & Addition of personnel who does not work for the organization performing requirements engineering activities. For example, end users, clients, external requirement experts. &  Ext \\
  \hline
Addition of Structure & Change in Environment by defining or creating standards or templates to accommodate certain process. For example, defining quality criteria or creating specification templates. &  AS \\
  \hline
Addition of New Role & Changes in Environment by defining appropriate roles and responsibilities among existing team members. For example, appointing a team leader or introducing manager. & AR \\
  \hline
  
   \end{tabular}
  % }

==> Tables/PeopleTable.tex <==
%\rotatebox{90}{
 \begin{tabular}{|p{.20\textwidth} | p{.65\textwidth} | p{.078\textwidth} | }
  \hline
\textbf{People} & \textbf{Description}& \textbf{Code}\\ 
  \hline
Internal Training Activities & Changes in People to improve their skills and performance such as communication skills or time management skills. This change occurs to the internal team members in a formal way. For example, planning and execution of trainings (in order to improve skill and performance)  & ITA \\
\hline
Internal Team Encouragement & Changes in People by encouraging the team as well as guiding them and making them aware of what needs to be done and how to do it right. This is an informal guidance to the internal team members. For example, Motivating team or empowering team; guiding team members to focus in customer requirements  & ITE \\
\hline
External Training and Coaching Activities & Changes in People induced by increasing awareness or guidance to external stake holders. This change occurs to the people external to the team, such as clients and customers in an informal way. For example, guiding client to understand that developers do not necessarily have domain knowledge; Training/Coaching/Consulting: Customers need to be held coached on the importance of this stage of software development and how much it costs in support and maintenance to do otherwise. &  ETA \\
  \hline
  
   \end{tabular}
  % }

==> Tables/ProcessTable.tex <==
 %\rotatebox{90}{
 \begin{tabular}{|p{.20\textwidth} | p{.65\textwidth} | p{.078\textwidth} | }
  \hline
\textbf{Process} & \textbf{Description} & \textbf{Code} \\ 
  \hline
Investigation & Changes in Process by identifying what to do and how to do to solve the problem occurred in the process. For example, evaluation of tools or identification of process gaps. It is not an exact process change, but investigation may cause change in process later. It will not solve the problem by itself but help try to identify what to do to solve the problem. & INV \\
  \hline
Refinement and Redesign & Changes in Process induced by - a) changes in Environment due to introduction of new processes, tools or approaches; b) refining or modifying the existing process as needed; or c) implementing existing process as a part of the process being modified. For Example, implementing a change management process, Prototypes and wire-frames to help developers understand the requirements, use of requirement quantification approach. & RR \\
  \hline
Definition of Roles and Responsibilities &  Changes in Process occurred by defining existing roles and responsibilities more clearly. & DR \\
  \hline
Resource Allocation & Changes in Process by allocating correct resources in correct events. For example, involving everyone representing every role in a software development project for requirement gathering process of that project. & RA \\
  \hline
   \end{tabular}
  % }
